Solving the Petri-Nets to Statecharts Transformation Case with UML-RSDS

This paper provides a solution to the Petri-Nets to statecharts case using UML-RSDS. We show how a highly declarative solution which is confluent and invertible can be given using this approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{101}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.13}{10.4204/EPTCS.135.13}}

